An Identification and Dimensionality Robust Test for Instrumental Variables Models

Using modifications of Lindeberg's interpolation technique, I propose a new identification-robust test for the structural parameter in a heteroskedastic instrumental variables model. While my analysis allows the number of instruments to be much larger than the sample size, it does not require many instruments, making my test applicable in settings that have not been well studied. Instead, the proposed test statistic has a limiting chi-squared distribution so long as an auxiliary parameter can be consistently estimated. This is possible using machine learning methods even when the number of instruments is much larger than the sample size. To improve power, a simple combination with the sup-score statistic of Belloni et al. (2012) is proposed. I point out that first-stage F-statistics calculated on LASSO selected variables may be misleading indicators of identification strength and demonstrate favorable performance of my proposed methods in both empirical data and simulation study.

==> misc/existing-tests.tex <==
\begin{table}[htbp!]
    \centering
    \begin{tabular}{|c|c|}
        \hline
        Asymptotic Regime & Main Tests\\
        \hline   
        % Low Dimensional Tests
        \begin{tabular}{@{}c@{}} \\ Low-Dimensional: \\ \(d_z^3/n \to 0\) \\ \hphantom{test} \end{tabular}       & 
        \begin{tabular}{@{}c@{}} \\ Anderson-Rubin \\ K/Lagrange Multiplier  \\ Conditional Linear Combination\\ \hphantom{test}\end{tabular} \\ 
        \hline 
        % Many Instrument Tests
        \begin{tabular}{@{}c@{}}
            \\ Many-Instruments: \\ \(d_z/n \to \phi \in [0,1)\) \\ \(d_z\to \infty\) \\ \hphantom{test}
        \end{tabular}  & 
        \begin{tabular}{@{}c@{}}
            Jackknife-AR \\ Jackknife-LM\\ Conditional Linear Combination \\ 
        \end{tabular} \\ 
        \hline
        % high-dimensional Tests 
        \begin{tabular}{@{}c@{}}
            \\ High-Dimensional: \\ \(\log^M(d_zn)/n\to 0\) \\ \hphantom{test}
        \end{tabular}
        &  
        \begin{tabular}{@{}c@{}}
            Sup-Score Test\\ Split-Sample AR         
        \end{tabular}
        \\
        \hline
    \end{tabular}
    \captionsetup{width=.625\linewidth, font = small}
    \caption{Existing Identification and Heteroskedasticity Robust Tests for Linear IV models.}
\end{table}



==> misc/power_plots.tex <==



==> misc/simulation_tables.tex <==
\begin{table}[htb!]
    \centering
    \begin{tabular}{|cccc|ccccccc|}
    \hline
    \multicolumn{4}{|c|}{\textbf{DGP}} & \multicolumn{7}{c|}{\textbf{Testing Procedure}} \\
    \rule{0pt}{0.1em} & & & & & & & & & &  \\
    \(n\) & \(d_z\) & \(\varrho_1\) & \(\varrho_2\) & \(\JK(\beta_0)\) & \(S(\beta_0)\) & \(T(\beta_0; \tau_{0.3})\) & \(T(\beta_0;\tau_{0.75})\) & A.Rbn. & JAR & JLM \\
    \hhline{|====|=======|}
    200 & 10 & 0.2 & 0.3 & 0.0516 & 0.0352 & 0.0406 & 0.0406 & 0.0296 & 0.0766 & 0.0502 \\ 
        &    & 0.2 & 0.6 & 0.0542 & 0.0306 & 0.0442 & 0.0384 & 0.0258 & 0.0748 & 0.0400 \\ 
        &    & 0.5 & 0.3 & 0.0470 & 0.0338 & 0.0416 & 0.0418 & 0.0238 & 0.0784 & 0.0460 \\ 
        &    & 0.5 & 0.6 & 0.0506 & 0.0350 & 0.0416 & 0.0390 & 0.0280 & 0.0676 & 0.0384 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 30 & 0.2 & 0.3 & 0.0570 & 0.0124 & 0.0422 & 0.0200 & 0.0088 & 0.1000 & 0.0382 \\ 
        &    & 0.2 & 0.6 & 0.0564 & 0.0126 & 0.0408 & 0.0208 & 0.0124 & 0.0962 & 0.0322 \\ 
        &    & 0.5 & 0.3 & 0.0498 & 0.0100 & 0.0366 & 0.0190 & 0.0096 & 0.1090 & 0.0318 \\ 
        &    & 0.5 & 0.6 & 0.0562 & 0.0118 & 0.0420 & 0.0216 & 0.0088 & 0.1104 & 0.0292 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 65 & 0.2 & 0.3 & 0.0542 & 0.0316 & 0.0428 & 0.0370 & 0.0314 & 0.0764 & 0.0420 \\ 
        &    & 0.2 & 0.6 & 0.0532 & 0.0366 & 0.0418 & 0.0398 & 0.0250 & 0.0780 & 0.0376 \\ 
        &    & 0.5 & 0.3 & 0.0474 & 0.0308 & 0.0388 & 0.0362 & 0.0244 & 0.0748 & 0.0354 \\ 
        &    & 0.5 & 0.6 & 0.0484 & 0.0324 & 0.0366 & 0.0388 & 0.0282 & 0.0708 & 0.0402 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
    500 & 10 & 0.2 & 0.3 & 0.0590 & 0.0468 & 0.0478 & 0.0516 & 0.0376 & 0.0652 & 0.0452 \\ 
        &    & 0.2 & 0.6 & 0.0530 & 0.0420 & 0.0460 & 0.0466 & 0.0366 & 0.0692 & 0.0434 \\ 
        &    & 0.5 & 0.3 & 0.0496 & 0.0370 & 0.0408 & 0.0368 & 0.0338 & 0.0710 & 0.0464 \\ 
        &    & 0.5 & 0.6 & 0.0512 & 0.0426 & 0.0456 & 0.0438 & 0.0334 & 0.0696 & 0.0404 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 30 & 0.2 & 0.3 & 0.0522 & 0.0202 & 0.0386 & 0.0278 & 0.0238 & 0.0818 & 0.0322 \\ 
        &    & 0.2 & 0.6 & 0.0558 & 0.0208 & 0.0408 & 0.0310 & 0.0266 & 0.0888 & 0.0342 \\ 
        &    & 0.5 & 0.3 & 0.0554 & 0.0178 & 0.0392 & 0.0280 & 0.0174 & 0.0940 & 0.0272 \\ 
        &    & 0.5 & 0.6 & 0.0570 & 0.0156 & 0.0426 & 0.0236 & 0.0206 & 0.0984 & 0.0280 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 65 & 0.2 & 0.3 & 0.0542 & 0.0372 & 0.0434 & 0.0432 & 0.0384 & 0.0754 & 0.0464 \\ 
        &    & 0.2 & 0.6 & 0.0584 & 0.0442 & 0.0482 & 0.0470 & 0.0334 & 0.0676 & 0.0438 \\ 
        &    & 0.5 & 0.3 & 0.0614 & 0.0460 & 0.0504 & 0.0496 & 0.0316 & 0.0708 & 0.0434 \\ 
        &    & 0.5 & 0.6 & 0.0526 & 0.0378 & 0.0434 & 0.0420 & 0.0298 & 0.0692 & 0.0358 \\ 
   \hline
   \end{tabular}
   \captionsetup{width = 0.95\linewidth, font = small}
   \caption{Simulated Size of Identification and Heteroskedasticity Robust Tests under Weak Identification. Each DGP is simulated 5000 times. Critical values of the sup-score statistic and quantiles of the conditioning statistic are calculated using 1000 multiplier bootstrap simulations.}
   \label{table:weak_size}
\end{table}
 
 
\begin{table}[htb!]
    \centering
    \begin{tabular}{|cccc|ccccccc|}
    \hline
    \multicolumn{4}{|c|}{\textbf{DGP}} & \multicolumn{7}{c|}{\textbf{Testing Procedure}} \\
    \rule{0pt}{0.1em} & & & & & & & & & &  \\
    \(n\) & \(d_z\) & \(\varrho_1\) & \(\varrho_2\) & \(\JK(\beta_0)\) & \(S(\beta_0)\) & \(T(\beta_0; \tau_{0.3})\) & \(T(\beta_0;\tau_{0.75})\) & A.Rbn. & JAR & JLM \\
    \hhline{|====|=======|}
    200 & 10 & 0.2 & 0.3 & 0.0474 & 0.0420 & 0.0474 & 0.0468 & 0.0308 & 0.0728 & 0.0424 \\ 
        &    & 0.2 & 0.6 & 0.0512 & 0.0386 & 0.0512 & 0.0506 & 0.0304 & 0.0764 & 0.0378 \\ 
        &    & 0.5 & 0.3 & 0.0416 & 0.0318 & 0.0414 & 0.0414 & 0.0248 & 0.0794 & 0.0428 \\ 
        &    & 0.5 & 0.6 & 0.0446 & 0.0342 & 0.0446 & 0.0442 & 0.0244 & 0.0806 & 0.0384 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 30 & 0.2 & 0.3 & 0.0482 & 0.0122 & 0.0448 & 0.0264 & 0.0110 & 0.1048 & 0.0370 \\ 
        &    & 0.2 & 0.6 & 0.0498 & 0.0120 & 0.0480 & 0.0312 & 0.0118 & 0.0980 & 0.0378 \\ 
        &    & 0.5 & 0.3 & 0.0456 & 0.0126 & 0.0410 & 0.0262 & 0.0082 & 0.1146 & 0.0268 \\ 
        &    & 0.5 & 0.6 & 0.0482 & 0.0110 & 0.0474 & 0.0308 & 0.0094 & 0.1090 & 0.0302 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 65 & 0.2 & 0.3 & 0.0528 & 0.0380 & 0.0526 & 0.0510 & 0.0276 & 0.0696 & 0.0460 \\ 
        &    & 0.2 & 0.6 & 0.0464 & 0.0360 & 0.0464 & 0.0468 & 0.0302 & 0.0728 & 0.0416 \\ 
        &    & 0.5 & 0.3 & 0.0482 & 0.0298 & 0.0480 & 0.0466 & 0.0246 & 0.0738 & 0.0412 \\ 
        &    & 0.5 & 0.6 & 0.0396 & 0.0320 & 0.0390 & 0.0386 & 0.0258 & 0.0748 & 0.0356 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
    500 & 10 & 0.2 & 0.3 & 0.0524 & 0.0444 & 0.0524 & 0.0524 & 0.0394 & 0.0684 & 0.0472 \\ 
        &    & 0.2 & 0.6 & 0.0476 & 0.0430 & 0.0476 & 0.0476 & 0.0400 & 0.0644 & 0.0490 \\ 
        &    & 0.5 & 0.3 & 0.0434 & 0.0410 & 0.0434 & 0.0434 & 0.0340 & 0.0702 & 0.0404 \\ 
        &    & 0.5 & 0.6 & 0.0448 & 0.0382 & 0.0448 & 0.0448 & 0.0350 & 0.0736 & 0.0432 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 30 & 0.2 & 0.3 & 0.0502 & 0.0214 & 0.0502 & 0.0498 & 0.0240 & 0.0854 & 0.0368 \\ 
        &    & 0.2 & 0.6 & 0.0522 & 0.0208 & 0.0522 & 0.0524 & 0.0224 & 0.0858 & 0.0392 \\ 
        &    & 0.5 & 0.3 & 0.0456 & 0.0202 & 0.0456 & 0.0434 & 0.0220 & 0.0918 & 0.0264 \\ 
        &    & 0.5 & 0.6 & 0.0500 & 0.0186 & 0.0500 & 0.0498 & 0.0204 & 0.0924 & 0.0268 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 65 & 0.2 & 0.3 & 0.0490 & 0.0426 & 0.0490 & 0.0490 & 0.0350 & 0.0742 & 0.0472 \\ 
        &    & 0.2 & 0.6 & 0.0522 & 0.0458 & 0.0522 & 0.0522 & 0.0436 & 0.0652 & 0.0442 \\ 
        &    & 0.5 & 0.3 & 0.0542 & 0.0476 & 0.0542 & 0.0542 & 0.0294 & 0.0712 & 0.0446 \\ 
        &    & 0.5 & 0.6 & 0.0438 & 0.0420 & 0.0438 & 0.0438 & 0.0306 & 0.0666 & 0.0500 \\ 
   \hline
   \end{tabular}
   \captionsetup{width = 0.95\linewidth, font = small}
   \caption{Simulated Size of Identification and Heteroskedasticity Robust Tests under Strong Identification. Each DGP is simulated 5000 times. Critical values of the sup-score statistic and quantiles of the conditioning statistic are calculated using 1000 multiplier bootstrap simulations.}
   \label{table:strong_size}
\end{table}


==> misc/simulation_tables_total.tex <==
\begin{table}[htbp!]
    \centering
    \begin{tabular}{|cccc|ccccccc|}
    \hline
    \multicolumn{4}{|c|}{\textbf{DGP}} & \multicolumn{7}{c|}{\textbf{Testing Procedure}} \\
    \rule{0pt}{0.1em} & & & & & & & & & &  \\
    \(n\) & \(d_z\) & \(\varrho_1\) & \(\varrho_2\) & \(\JK(\beta_0)\) & \(S(\beta_0)\) & \(T(\beta_0; \tau_{0.3})\) & \(T(\beta_0;\tau_{0.75})\) & A.Rbn. & JAR & JLM \\
    \hhline{|====|=======|}
    200 & 10 & 0.2 & 0.3 & 0.0516 & 0.0352 & 0.0406 & 0.0406 & 0.0296 & 0.0766 & 0.0502 \\ 
        &    & 0.2 & 0.6 & 0.0542 & 0.0306 & 0.0442 & 0.0384 & 0.0258 & 0.0748 & 0.0400 \\ 
        &    & 0.5 & 0.3 & 0.0470 & 0.0338 & 0.0416 & 0.0418 & 0.0238 & 0.0784 & 0.0460 \\ 
        &    & 0.5 & 0.6 & 0.0506 & 0.0350 & 0.0416 & 0.0390 & 0.0280 & 0.0676 & 0.0384 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 30 & 0.2 & 0.3 & 0.0570 & 0.0124 & 0.0422 & 0.0200 & 0.0088 & 0.1000 & 0.0382 \\ 
        &    & 0.2 & 0.6 & 0.0564 & 0.0126 & 0.0408 & 0.0208 & 0.0124 & 0.0962 & 0.0322 \\ 
        &    & 0.5 & 0.3 & 0.0498 & 0.0100 & 0.0366 & 0.0190 & 0.0096 & 0.1090 & 0.0318 \\ 
        &    & 0.5 & 0.6 & 0.0562 & 0.0118 & 0.0420 & 0.0216 & 0.0088 & 0.1104 & 0.0292 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 65 & 0.2 & 0.3 & 0.0542 & 0.0316 & 0.0428 & 0.0370 & 0.0314 & 0.0764 & 0.0420 \\ 
        &    & 0.2 & 0.6 & 0.0532 & 0.0366 & 0.0418 & 0.0398 & 0.0250 & 0.0780 & 0.0376 \\ 
        &    & 0.5 & 0.3 & 0.0474 & 0.0308 & 0.0388 & 0.0362 & 0.0244 & 0.0748 & 0.0354 \\ 
        &    & 0.5 & 0.6 & 0.0484 & 0.0324 & 0.0366 & 0.0388 & 0.0282 & 0.0708 & 0.0402 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 75 & 0.2 & 0.3 & 0.0512 & 0.0122 & 0.0364 & 0.0210 & 0.0150 & 0.0972 & 0.0422 \\ 
        &    & 0.2 & 0.6 & 0.0564 & 0.0162 & 0.0416 & 0.0272 & 0.0152 & 0.0974 & 0.0414 \\ 
        &    & 0.5 & 0.3 & 0.0488 & 0.0136 & 0.0368 & 0.0208 & 0.0168 & 0.1144 & 0.0380 \\ 
        &    & 0.5 & 0.6 & 0.0516 & 0.0128 & 0.0390 & 0.0224 & 0.0122 & 0.1166 & 0.0390 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
    500 & 10 & 0.2 & 0.3 & 0.0590 & 0.0468 & 0.0478 & 0.0516 & 0.0376 & 0.0652 & 0.0452 \\ 
        &    & 0.2 & 0.6 & 0.0530 & 0.0420 & 0.0460 & 0.0466 & 0.0366 & 0.0692 & 0.0434 \\ 
        &    & 0.5 & 0.3 & 0.0496 & 0.0370 & 0.0408 & 0.0368 & 0.0338 & 0.0710 & 0.0464 \\ 
        &    & 0.5 & 0.6 & 0.0512 & 0.0426 & 0.0456 & 0.0438 & 0.0334 & 0.0696 & 0.0404 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 30 & 0.2 & 0.3 & 0.0522 & 0.0202 & 0.0386 & 0.0278 & 0.0238 & 0.0818 & 0.0322 \\ 
        &    & 0.2 & 0.6 & 0.0558 & 0.0208 & 0.0408 & 0.0310 & 0.0266 & 0.0888 & 0.0342 \\ 
        &    & 0.5 & 0.3 & 0.0554 & 0.0178 & 0.0392 & 0.0280 & 0.0174 & 0.0940 & 0.0272 \\ 
        &    & 0.5 & 0.6 & 0.0570 & 0.0156 & 0.0426 & 0.0236 & 0.0206 & 0.0984 & 0.0280 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 65 & 0.2 & 0.3 & 0.0542 & 0.0372 & 0.0434 & 0.0432 & 0.0384 & 0.0754 & 0.0464 \\ 
        &    & 0.2 & 0.6 & 0.0584 & 0.0442 & 0.0482 & 0.0470 & 0.0334 & 0.0676 & 0.0438 \\ 
        &    & 0.5 & 0.3 & 0.0614 & 0.0460 & 0.0504 & 0.0496 & 0.0316 & 0.0708 & 0.0434 \\ 
        &    & 0.5 & 0.6 & 0.0526 & 0.0378 & 0.0434 & 0.0420 & 0.0298 & 0.0692 & 0.0358 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 75 & 0.2 & 0.3 & 0.0522 & 0.0234 & 0.0428 & 0.0316 & 0.0280 & 0.0818 & 0.0430 \\ 
        &    & 0.2 & 0.6 & 0.0518 & 0.0252 & 0.0412 & 0.0318 & 0.0274 & 0.0916 & 0.0422 \\ 
        &    & 0.5 & 0.3 & 0.0500 & 0.0240 & 0.0400 & 0.0316 & 0.0274 & 0.1028 & 0.0470 \\ 
        &    & 0.5 & 0.6 & 0.0522 & 0.0220 & 0.0434 & 0.0328 & 0.0230 & 0.1002 & 0.0434 \\ 
   \hline
   \end{tabular}
   \captionsetup{width = 0.95\linewidth, font = small}
   \caption{Simulated Size of Identification and Heteroskedasticity Robust Tests under Weak Identification. Each DGP is simulated 5000 times. Critical values of the sup-score statistic and quantiles of the conditioning statistic are calculated using 1000 multiplier bootstrap simulations.}
   \label{table:weak_size_total}
\end{table}
 
 
\begin{table}[htbp!]
    \centering
    \begin{tabular}{|cccc|ccccccc|}
    \hline
    \multicolumn{4}{|c|}{\textbf{DGP}} & \multicolumn{7}{c|}{\textbf{Testing Procedure}} \\
    \rule{0pt}{0.1em} & & & & & & & & & &  \\
    \(n\) & \(d_z\) & \(\varrho_1\) & \(\varrho_2\) & \(\JK(\beta_0)\) & \(S(\beta_0)\) & \(T(\beta_0; \tau_{0.3})\) & \(T(\beta_0;\tau_{0.75})\) & A.Rbn. & JAR & JLM \\
    \hhline{|====|=======|}
    200 & 10 & 0.2 & 0.2 & 0.0474 & 0.0420 & 0.0474 & 0.0468 & 0.0308 & 0.0728 & 0.0424 \\ 
        &    & 0.2 & 0.6 & 0.0512 & 0.0386 & 0.0512 & 0.0506 & 0.0304 & 0.0764 & 0.0378 \\ 
        &    & 0.5 & 0.2 & 0.0416 & 0.0318 & 0.0414 & 0.0414 & 0.0248 & 0.0794 & 0.0428 \\ 
        &    & 0.5 & 0.6 & 0.0446 & 0.0342 & 0.0446 & 0.0442 & 0.0244 & 0.0806 & 0.0384 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 30 & 0.2 & 0.2 & 0.0482 & 0.0122 & 0.0448 & 0.0264 & 0.0110 & 0.1048 & 0.0370 \\ 
        &    & 0.2 & 0.6 & 0.0498 & 0.0120 & 0.0480 & 0.0312 & 0.0118 & 0.0980 & 0.0378 \\ 
        &    & 0.5 & 0.2 & 0.0456 & 0.0126 & 0.0410 & 0.0262 & 0.0082 & 0.1146 & 0.0268 \\ 
        &    & 0.5 & 0.6 & 0.0482 & 0.0110 & 0.0474 & 0.0308 & 0.0094 & 0.1090 & 0.0302 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 65 & 0.2 & 0.2 & 0.0528 & 0.0380 & 0.0526 & 0.0510 & 0.0276 & 0.0696 & 0.0460 \\ 
        &    & 0.2 & 0.6 & 0.0464 & 0.0360 & 0.0464 & 0.0468 & 0.0302 & 0.0728 & 0.0416 \\ 
        &    & 0.5 & 0.2 & 0.0482 & 0.0298 & 0.0480 & 0.0466 & 0.0246 & 0.0738 & 0.0412 \\ 
        &    & 0.5 & 0.6 & 0.0396 & 0.0320 & 0.0390 & 0.0386 & 0.0258 & 0.0748 & 0.0356 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 75 & 0.2 & 0.2 & 0.0516 & 0.0120 & 0.0498 & 0.0406 & 0.0188 & 0.1070 & 0.0414 \\ 
        &    & 0.2 & 0.6 & 0.0444 & 0.0130 & 0.0436 & 0.0392 & 0.0198 & 0.1052 & 0.0408 \\ 
        &    & 0.5 & 0.2 & 0.0416 & 0.0100 & 0.0408 & 0.0328 & 0.0128 & 0.1094 & 0.0412 \\ 
        &    & 0.5 & 0.6 & 0.0480 & 0.0128 & 0.0474 & 0.0432 & 0.0122 & 0.1096 & 0.0430 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
    500 & 10 & 0.2 & 0.2 & 0.0524 & 0.0444 & 0.0524 & 0.0524 & 0.0394 & 0.0684 & 0.0472 \\ 
        &    & 0.2 & 0.6 & 0.0476 & 0.0430 & 0.0476 & 0.0476 & 0.0400 & 0.0644 & 0.0490 \\ 
        &    & 0.5 & 0.2 & 0.0434 & 0.0410 & 0.0434 & 0.0434 & 0.0340 & 0.0702 & 0.0404 \\ 
        &    & 0.5 & 0.6 & 0.0448 & 0.0382 & 0.0448 & 0.0448 & 0.0350 & 0.0736 & 0.0432 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 30 & 0.2 & 0.2 & 0.0502 & 0.0214 & 0.0502 & 0.0498 & 0.0240 & 0.0854 & 0.0368 \\ 
        &    & 0.2 & 0.6 & 0.0522 & 0.0208 & 0.0522 & 0.0524 & 0.0224 & 0.0858 & 0.0392 \\ 
        &    & 0.5 & 0.2 & 0.0456 & 0.0202 & 0.0456 & 0.0434 & 0.0220 & 0.0918 & 0.0264 \\ 
        &    & 0.5 & 0.6 & 0.0500 & 0.0186 & 0.0500 & 0.0498 & 0.0204 & 0.0924 & 0.0268 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 65 & 0.2 & 0.2 & 0.0490 & 0.0426 & 0.0490 & 0.0490 & 0.0350 & 0.0742 & 0.0472 \\ 
        &    & 0.2 & 0.6 & 0.0522 & 0.0458 & 0.0522 & 0.0522 & 0.0436 & 0.0652 & 0.0442 \\ 
        &    & 0.5 & 0.2 & 0.0542 & 0.0476 & 0.0542 & 0.0542 & 0.0294 & 0.0712 & 0.0446 \\ 
        &    & 0.5 & 0.6 & 0.0438 & 0.0420 & 0.0438 & 0.0438 & 0.0306 & 0.0666 & 0.0500 \\ 
    \rule{0pt}{0.1em} & & & & & & & & & &  \\ 
        & 75 & 0.2 & 0.2 & 0.0480 & 0.0220 & 0.0480 & 0.0480 & 0.0314 & 0.0880 & 0.0394 \\ 
        &    & 0.2 & 0.6 & 0.0492 & 0.0284 & 0.0492 & 0.0492 & 0.0278 & 0.0874 & 0.0470 \\ 
        &    & 0.5 & 0.2 & 0.0404 & 0.0190 & 0.0404 & 0.0404 & 0.0254 & 0.0992 & 0.0426 \\ 
        &    & 0.5 & 0.6 & 0.0470 & 0.0226 & 0.0470 & 0.0468 & 0.0182 & 0.0960 & 0.0418 \\ 
   \hline
   \end{tabular}
   \captionsetup{width = 0.95\linewidth, font = small}
   \caption{Simulated Size of Identification and Heteroskedasticity Robust Tests under Strong Identification. Each DGP is simulated 5000 times. Critical values of the sup-score statistic and quantiles of the conditioning statistic are calculated using 1000 multiplier bootstrap simulations.}
   \label{table:strong_size_total}
\end{table}


==> misc/varphi_graph.tex <==
\usetikzlibrary{arrows.meta}
\begin{figure}
\begin{center}
    \begin{tikzpicture}
        \draw[gray, ultra thin] (-0.6,-0.075) grid[xstep = 0.75, ystep = 0.75] (4.35,3.6);
        \draw[-stealth, thick] (-0.75,0) -- (4.5,0) node[right] {$x$};
        \draw[-stealth, thick] (0,-0.15) -- (0,3.75) node[above] {$y$};
        \draw[scale=3, domain= -0.25:0, smooth, variable = \x, blue, thick] plot ({\x} , {1}); 
        \draw[scale=3, domain= 0:1, smooth, variable = \x, blue, thick] plot ({\x} , {1 - 140*(0.25*\x^4 - 0.6*\x^5 + 0.5*\x^6 - (1/7)*\x^7)}); 
        \draw[scale=3, domain= 1:1.45, smooth, variable = \x, blue, thick] plot ({\x} , {0}) node[above left] {$\varphi_\gamma(x)$}; 
        \draw[stealth-stealth, red, thick] (0.075,1.5) -- (1.425,1.5) node[above right] {$\gamma = 1$};
        % Arrow between plots
        \draw[-{Triangle[open]}, thick] (4.875,1.5) -- (6.375,1.5) ;
        %New plot
        \draw[gray, ultra thin] (6.9,-0.075) grid[xstep = 0.75, ystep = 0.75] (11.85,3.6);
        \draw[-stealth, thick] (6.75,0) -- (12,0) node[right] {$x$};
        \draw[-stealth, thick] (7.5,-0.16) -- (7.5,3.75) node[above] {$y$};
        \draw[scale=3, domain= 2.25:2.5, smooth, variable = \x, blue, thick] plot ({\x} , {1}); 
        \draw[scale=3, domain= 2.5:3, smooth, variable = \x, blue, thick] plot ({\x} , {1 - 140*(0.25*((\x-2.5)/0.5)^4 - 0.6*((\x-2.5)/0.5)^5 + 0.5*((\x-2.5)/0.5)^6 - (1/7)*((\x-2.5)/0.5)^7)}); 
        \draw[scale=3, domain= 3:3.95, smooth, variable = \x, blue, thick] plot ({\x} , {0}) node[above left] {$\varphi_\gamma(x)$}; 
        \draw[stealth-stealth, red, thick] (7.575,1.5) -- (8.175,1.5) node[above right] {$\gamma = 0.5$};
    \end{tikzpicture}
\end{center}
\captionsetup{width=.72\linewidth, font = small}
\caption{The functions \(\varphi_{\gamma}(x)\) approximate the indicator \(\bm{1}\{x \leq 0\}\) from above. The quality of approximation increases as the parameter \(\gamma\) tends to zero, but the second and third derivatives increase on the order of \(\gamma^{-2}\) and \(\gamma^{-3}\), respectively.}
\label{fig:varphi-approximation}
\end{figure}


==> sections/multiple_endogeneous.tex <==
\section[Multiple Endogenous Variables]{Limiting Behavior of Test Statistic}
\label{sec:multiple-endogeneous}

To analyze the limiting behavior of the test statistic when I show that quantiles of the jackknife K-statistic can be approximated by analogous quantiles of the Gaussian statistic:
\[
    \JK_G(\beta_0) \coloneqq \tilde\eps(\beta_0)\tilde\Pi(\tilde\Pi_\eps' \tilde\Pi_\eps)^{-1}\tilde\Pi'\tilde\eps(\beta_0);
\]
where \((\tilde\eps_i(\beta_0),\tilde r_i)'\) are Gaussian with the same mean and covariance matrix as \((\eps_i(\beta_0),r_i)'\) and for \(\tilde\Pi_{\ell i} = \sum_{j\neq i} h_{ij} \tilde r_{\ell j}\) define \(\tilde\Pi_i \coloneqq (\tilde\Pi_{1i},\dots,\tilde\Pi_{d_xi})'\in\SR^{d_x}\), \(\tilde\Pi_{\eps i} \coloneqq (\E[\eps_i^2(\beta_0)])^{1/2}\tilde\Pi_i\),
\begin{align*}
    \tilde\eps(\beta_0) 
    &\coloneqq (\tilde\eps_1(\beta_0),\dots,\tilde\eps_n(\beta_0))' \in \SR^n,\\ 
    \tilde\Pi &\coloneqq (\tilde\Pi_1,\dots,\tilde\Pi_n)' \in \SR^{n\times d_x},\\ 
    \text{and }\;\tilde\Pi_\eps &\coloneqq (\tilde\Pi_{\eps 1},\dots,\tilde\Pi_{\eps n})' \in \SR^{n\times d_x}.
\end{align*}
As uncorrelated jointly Gaussian random variables are independent, under \(H_0\) the vector \(\tilde\eps(\beta_0)\) is mean zero and independent of \((\tilde\Pi, \tilde\Pi_\eps)\). Conditional on any realization of \((\tilde\Pi,\tilde\Pi_\eps)\) the \(\JK_G(\beta_0)\) statistic then follows a \(\chi^2_{d_x}\) distribution, and thus, its unconditional distribution is also \(\chi^2_{d_x}\).
As before, error taken on from the estimation of \(\rho(z_i)\) prevents immediate comparison of \(\JK(\beta_0)\) to \(\JK_G(\beta_0)\) so I begin by showing that the quantiles of an infeasible statistic, \(\JK_I(\beta_0)\), can be approximated by corresponding quantiles of \(\JK_G(\beta_0)\) where:
\[
    \JK_I(\beta_0) \coloneqq \eps(\beta_0)(\widehat\Pi^I)((\widehat\Pi_\eps^I)'(\widehat\Pi_{\eps}^I))^{-1}(\widehat\Pi^I)'\eps(\beta_0),
\]
for \(\widehat\Pi^I\) and \(\widehat\Pi_{\eps}^I\) defined the same way as \(\widehat\Pi\) and \(\widehat\Pi_\eps\) in \eqref{eq:hatPi-hatPiEps}, respectively, but using the true values \((r_1,\dots,r_n)'\) in place of their estimates \((\hat r_1,\dots,\hat r_n)'\).

When there are multiple endogenous variables, \(d_x > 1\), I cannot take advantage of the simplified form of the test statistic to establish this approximation as in \Cref{sec:single-endogeneous}. Instead I deal directly with the test statistics themselves. Consider functions \(\varphi_\gamma(\cdot) \in C_b^3(\SR)\) that approximate the indicators \(\bm{1}\{\cdot \leq a\}\), where \(a \in \SR\) is arbitrary and \(\gamma\) is a scaling factor inversely proportional to the quality of the approximation but positively proportional to the derivatives of \(\varphi_\gamma\). The goal is to show, for a sequence \(\gamma_n\) tending to zero, that
\begin{equation}
    \label{eq:multiple-goal}
    \E[\varphi_{\gamma_n}(\JK_I(\beta_0)) - \varphi_{\gamma_n}(\JK_G(\beta_0))] \to 0
\end{equation}
As mentioned in \Cref{sec:single-endogeneous}, the Lindeberg's original approach cannot be applied the derivative of the test statistics with respect to terms in the denominator matrix, \(\widehat\Pi_\eps'\widehat\Pi_\eps\), may be as large as the inverse of the minimum eigenvalue of the denominator matrix. When identification is sufficiently weak, the denominator matrix will have a nonnegligible distribution and the inverse of its minimum eigenvalue may not have finite moments. 

To get around this, I modify the argument by considering a ``data-dependent'' choice of approximation parameter \(\gamma_n\). This choice of approximation parameter inversely scales with the determinant of the denominator matrix and thus, since the determinant is the product of the eigenvalues, inversely scales with the minimum eigenvalue.\footnote{The determinant has the benefit of being a smooth function of elements of the matrix. This makes it nicer to work with than the minimum eigenvalue itself, which loses differentiability when the dimension of its eigenspace is larger than one.} Geometrically, this approach can be thought of as ``stretching out'' the function \(\varphi_{\gamma_n}(\cdot)\) in directions where the minimum eigenvalue of the denominator matrix is close to zero. Through the chain rule, this allows for control of the overall derivative of \(\varphi_{\gamma_n}(\JK_I(\beta_0))\) with respective to an
individual observation. 
% Since the overall derivatives of \(\varphi_{\gamma_n}(\JK_I(\beta_0))\) with respect to \((\eps_i(\beta_0),r_i)'\) depend on the product of derivatives with respect to the test statistic and derivatives of \(\varphi_{\gamma_n}(\cdot)\), which scale inversely with the approximation parameter, this adjustment of the approximation parameter allows control of the overall derivative.

This approach relies on stronger moment conditions, needed mainly needed to bound moments of the determinant of the denominator matrix. For all \(\ell = 1,\dots,d_x\) let \(\zeta_{\ell i} \coloneqq v_i - \rho_\ell(z_i)\eta_i\) and \(\eta_i = \eps_i - v_i'(\beta - \beta_0)\), the demeaned versions of \(r_{\ell i}\) and \(\eps_i(\beta_0)\), respectively.
\begin{assumption}[Moment Conditions]
    \label{assm:multiple-moment-bounds}
    Assume (i) there are constants \(c > 1\) and \(\upsilon \in (0,1]\cup\{2\}\) such that \(\|\eps_i\|_{\psi_a} \leq c\) and \(\|\zeta_{\ell i}\|_{\psi_\upsilon} \leq c\), and (ii) \(c^{-1} \leq \lambda_{\min}(\E[\eta_i\eta_i']) \leq \lambda_{\max}(\E[\eta_i\eta_i']) \leq c\).
\end{assumption}

\begin{assumption}[Balanced Design]
    \label{assm:multiple-balanced-design}
    (i) Let \(s_{\ell, n}^{-2} = \max_{1 \leq i \leq n}\E[(\widehat\Pi_{\ell i}^I)^2]\) for each \(\ell \in [d_x]\); then, the minimum eigenvalue of the following matrix is bounded away from zero:
    \[
        c^{-1} \leq \lambda_{\min}\E\begin{pmatrix} \frac{s_{\ell,n}s_{k,n}}{n}\sum_{i=1}^n (\widehat\Pi_{\ell i}^I)(\widehat\Pi_{k i}^I) \end{pmatrix}_{\substack{1 \leq \ell \leq d_x \\ 1 \leq k \leq d_x}}
    \] 
    (ii) \(\max_i s_n \sum_{j\neq i} h_{ji}^2 \leq c\); and 
    (iii)  the following ratio is bounded away from zero: \(\frac{\sum_{k=2}^n\lambda_k^2(HH')}{\sum_{k=1}^n\lambda_k^2(HH')} \geq c^{-1}\) where \(\lambda_k(HH')\) represents the \(k^{\text{th}}\) largest eigenvalue of the matrix \(HH'\). 
\end{assumption}
\Cref{assm:multiple-moment-bounds}(i) strengthens \Cref{assm:moment-assumptions} to require that the random variables \((\eta_i,\zeta_i)\), and thus, by extension, \((\eps_i(\beta_0),r_i)\) are \(\upsilon\)-sub-exponential. As discussed below \Cref{assm:estimation-error} this is more restrictive than the finite sixth moments needed to establish \Cref{thm:local-power} but still allows for a wide range of possible distributions. \Cref{assm:multiple-moment-bounds}(ii) is a light regularity condition requiring that the random variables \((\eta_{1i},\dots,\eta_{d_x i})\) be linearly independent.

\Cref{assm:multiple-balanced-design}(i) is a natural extension of \Cref{assm:balanced-design}(i) to the setting where \(d_x > 1\). It requires that the average second moment of any linear combination of the first-stage estimates is proportional to the maximum second moment of the same linear combination. \Cref{assm:multiple-balanced-design}(ii,iii) are the same conditions as \Cref{assm:balanced-design}(ii,iii) and can again be implicitly thought of as requiring that the maximum leverage of any one observation be bounded and there be than two effective instruments in the hat matrix. \Cref{assm:multiple-balanced-design} thus reduces to \Cref{assm:balanced-design} when \(d_x = 1\).

Finally, two assumptions are needed to define the local neighborhoods considered and to show that estimation error can be treated as negligible when using the \(\ell_1\)-penalized procedure detailed in \Cref{sec:setup}. These assumptions are the natural extensions \Cref{assm:local-identification} and \Cref{assm:estimation-error}, respectively, and the reader is thus referred to \Cref{sec:single-endogeneous} for a discussion of their interpretations.

\begin{assumption}[Local Identification]
    \label{assm:multiple-local-identification}
    (i) The local power index is bounded \(P \leq c\) for
    \[
        P = \sum_{\ell = 1}^{d_x} \E\bigg[\bigg(\frac{s_{\ell,n}}{\sqrt{n}}\sum_{i=1}^n \widehat\Pi_{\ell i}^I\Pi_i'(\beta - \beta_0)\bigg)^2\bigg]
    \]
    (ii) \(\E[(s_{n,\ell}\sum_{j\neq i} h_{ji} \eps_j(\beta_0))^2] \leq c\) for all \(\ell = 1,\dots,d_x\).
\end{assumption}

\begin{assumption}[Estimation Error]
    \label{assm:multiple-estimation-error}
    (i) The basis terms \(b(z_i)\) are bounded, \(\|b(z_i)\|_\infty \leq C\) for all \(i =1,\dots,n\); (ii) the approximation error satisfies \((\E_n[\xi_{\ell i}^2])^{1/2} = o(n^{-1/2})\); (iii) the researcher has access to estimators \(\widehat\phi_\ell\) of \(\phi_\ell\) that satisfy \(\log(d_b n)^{2/(\upsilon\wedge 1)}\|\widehat\phi_\ell - \phi_\ell\|_1 \to_p 0\) for each \(\ell \in [d_x]\); and (iv) locally identified in the sense that
    \begin{enumerate}
        \item[(iva)] \(\max_{\substack{1 \leq \ell \leq d_x \\ 1 \leq k \leq d_b}} \big|\E\big[\frac{s_{n,\ell}}{\sqrt{n}}\sum_{i=1}^n \sum_{j\neq i}  h_{ij}\eps_i(\beta_0)b_k(z_j)\eps_j(\beta_0)\big]\big| \leq c \)
        \item[(ivb)] \(\max_{\substack{1 \leq i \leq n \\ 1 \leq \ell \leq d_b}} |\E[s_{n,\ell}\sum_{j\neq i} h_{ij}b_\ell(z_j)\eps_j(\beta_0)]| \leq c.\)
    \end{enumerate}
\end{assumption}

With these stated, I show that the results of \Cref{sec:single-endogeneous} can be extended to the general case. 
\begin{theorem}[Uniform Approximation]
    \label{thm:multiple-feasible-local-power}
    Suppose that \Cref{assm:multiple-moment-bounds,assm:multiple-balanced-design,assm:multiple-local-identification,assm:multiple-estimation-error} hold. Then,
    \[
        \sup_{a\in\SR}|\Pr(\JK(\beta_0) \leq a) - \Pr(\JK_G(\beta_0) \leq a)|\to 0
    \]
    In particular, under \(H_0\), \(\JK(\beta_0)\rightsquigarrow \chi^2_{d_x}\).
\end{theorem}
As discussed in \Cref{subsec:power-analysis}, tests based on the jackknife K-statistic may suffer from suboptimal power properties against certain alternatives. The power decline is particularly prnounced whenever \(\E[\widehat\Pi_{\ell i}] =  0\) for some \(\ell \in [d_x]\) and all \(i \in [n]\). To improve power in this direction, I propose a generalization of the thresholding test in \Cref{subsec:combination-test} based on the conditioning statistic \(C\)
\begin{align}
    \label{eq:multiple-conditioning}
    C \coloneqq \min_{1 \leq \ell \leq d_x} \max_{1 \leq i \leq n}\bigg| \frac{\sum_{j\neq i} h_{ij}\hat r_{\ell j}}{(\sum_{j\neq i} h_{ij}^2)^{1/2}}\bigg|
\end{align}
The conditioning statistic \(C\) attempts to detect whether, for \emph{some} \(\ell \in [d_x]\), \(\E[\widehat\Pi_{\ell i}^I] = 0\) for all \(i \in [n]\). Under the assumption that \(\E[\widehat\Pi_{\ell i}^I] = 0, \forall i \in [n], \ell \in [d_x]\), quantiles of \(C\) can be simulated by multiplier bootstrap. Let \(e_1,\dots,e_n\) be generated iid standard normal independent of the data and for any \(\theta\in (0,1)\), define the conditional bootstrap quantile:
\[
    c^C_{1-\theta} \coloneqq(1 -\theta)\text{ quantile of } \min_{1 \leq \ell \leq d_x} \max_{1 \leq i \leq n} \bigg|\frac{\sum_{j\neq i} e_jh_{ij}\hat r_j}{(\sum_{j\neq i} h_{ij}^2)^{1/2}}\bigg|\text{ conditional on }\{(y_i,x_i,z_i)\}_{i=1}^n 
\]
Based on the value of the conditioning statistic the researcher can decide whether to run a test based on \(\JK(\beta_0)\) or a test based on the sup-score statistic \(S(\beta_0)\).
\begin{align}
    \label{eq:multiple-thresholding-statistic}
    T(\beta_0;\tau) \coloneqq
    \begin{cases}
        \bm{1}\{\JK(\beta_0) > \chi^2_{d_x;1-\alpha}\} &\text{if } C > \tau \\
        \bm{1}\{S(\beta_0) > c^S_{1-\alpha}\} &\text{if } C \leq \tau
    \end{cases}
\end{align}
As with \Cref{thm:joint-combination}, I show the asymptotic validity of the thresholding test by first establishing that quantiles of \((\JK(\beta_0),C)\) and \((S(\beta_0),C)\) can jointly be approximated by Gaussian analogs and then using the marginal independence of the Gaussian analog testing and conditioning statistics under the null; \((\JK(\beta_0)\perp C)\) and \((S\beta_0)\perp C)\) under \(H_0\).
\begin{theorem}[]
    \label{thm:multiple-thresholding-alpha}
    Suppose that Assumptions \ref{assm:comb-conditions}(ii,iii), \ref{assm:multiple-moment-bounds}, \ref{assm:multiple-balanced-design}, and \ref{assm:multiple-estimation-error} hold. Then,
    \begin{enumerate}
        \item the test based on \(T(\beta_0;\tau)\) has asymptotic size \(\alpha\) for any choice of cutoff \(\tau\), and 
        \item if \(\E[\widehat\Pi_{\ell i}^I] = 0\) for all \(i \in [n]\) and \(\ell \in [d_x]\), there exist sequences \(\delta_n \searrow 0\) and \(\beta_n \searrow 0\) such that with probability at least \(1 - \delta_n\),
        \[
            \sup_{\theta\in (0,1)}|\Pr_e(C \leq c_{1-\theta}^C) - (1-\theta)| \leq \beta_n
        \]
        where \(\Pr_e(\cdot)\) denotes the probability with respect to only the variables \(e_1,\dots,e_n\).
    \end{enumerate}
\end{theorem}
The first part of \Cref{thm:multiple-thresholding-alpha} establishes the validity of the test based on the thresholding statistic for any choice of cutoff \(\tau\). In practice, I recommend taking the cutoff, \(\tau\), to be the 75\textsuperscript{th} quantile of the distribution of \(C\) under the assumption that \(\E[\widehat\Pi_{\ell i}^I] = 0\) for all \(\ell \in [d_x]\) and \(i \in [n]\). The second part of \Cref{thm:multiple-thresholding-alpha} establishes that this quantile can be simulated via the multiplier bootstrap procedure described above.


